DLWIoT: Deep Learning-based Watermarking for Authorized IoT Onboarding

The onboarding of IoT devices by authorized users constitutes both a challenge and a necessity in a world, where the number of IoT devices and the tampering attacks against them continuously increase. Commonly used onboarding techniques today include the use of QR codes, pin codes, or serial numbers. These techniques typically do not protect against unauthorized device access-a QR code is physically printed on the device, while a pin code may be included in the device packaging. As a result, any entity that has physical access to a device can onboard it onto their network and, potentially, tamper it (e.g.,install malware on the device). To address this problem, in this paper, we present a framework, called Deep Learning-based Watermarking for authorized IoT onboarding (DLWIoT), featuring a robust and fully automated image watermarking scheme based on deep neural networks. DLWIoT embeds user credentials into carrier images (e.g., QR codes printed on IoT devices), thus enables IoT onboarding only by authorized users. Our experimental results demonstrate the feasibility of DLWIoT, indicating that authorized users can onboard IoT devices with DLWIoT within 2.5-3sec.

==> discussion.tex <==
Using QR code to design and implement a e-shopping systems for smart mobile phone. 
\sol can be

\TODO{Peggy, can you write some discussion on how we could potentially have this model run directly on a mobile phone? I will add some discussion on some security/networking aspects.}



\TODO{Spyros: Talk about cases that users sell their IoT devices. How these devices will be able to get onboarded by new users?}

==> usecase.tex <==
The onboarding of IoT devices has been a major challenge, especially when security becomes a requirement. One of the common techniques for IoT onboarding today is the use of QR codes (other popular out-of-band IoT onboarding techniques include the use pin codes or serial numbers)~\cite{latvala2020evaluation}. A user scans the QR code of an IoT device with his/her mobile phone and this QR code is translated to a url, which allows the user to communicate with a server typically located on the cloud. Through this process, an IoT device acquires the necessary configuration and credentials, so that they onboard the user IoT network (\ie become an operational part of this network).

However, this onboarding technique does not protect against unauthorized use from the moment that an IoT device is manufactured until the time that a legitimate user tries to onboarding this device. For example, unauthorized users or any other entity that has physical access to the IoT device can onboarding it onto their personal network. As a result, an attacker could tamper the device (\eg by installing malicious software on it).

To protect against unauthorized onboarding, image watermarking techniques can be leveraged. Users order their IoT devices from a trusted party (\eg manufacturer), while this trusted party embeds a watermark instructed by the user (\eg user credentials) covertly onto a carrier image (\eg QR code). The marked image (\ie the watermark embedded into the carrier image) is printed on the device or is transmitted back to the user through a secure connection (\eg the image can be accessed by the user through a mobile application provided by the trusted party). When the user receives the ``watermarked'' IoT device, this image will be used for the on-boarding of the device onto the user network. Specifically, the user will take a picture of the image with his/her mobile phone (or access the image through a mobile application), the watermark will be extracted, and the device will be on-boarded. Note that only the authorized user will be able to extract the watermark and on-board the device. Attackers will not be able to on-board and tamper the device even if they have physical access to it, assuming that they do not have access to the user credentials used for the creation of the watermark.

\noindent \textbf{Why using deep learning for watermarking:} \TODO{Xin review here: 1. Maunal limitation => automation, 2. high robustness without prior knowledge}Among the goals of an image watermarking system is robustness--the watermark must survive even after distortion or quality degradation of the marked image~\cite{cox2007digital}. This is especially needed when a marked image is printed on a device and/or the embedded watermark is extracted from images captured by a mobile phone. To this end, a deep learning model for watermarking can provide enhanced robustness during the process of embedding a watermark to a marked image and extracting the watermark from camera resamples of a marked image, being able to deal with different degrees of distortion and image quality degradation, such as lighting variations, compression, and lens distortion~\cite{pramila2007camera}.

Moreover, conventional watermarking schemes are based on fixed algorithms for watermark embedding and extraction. A deep learning model can dynamically learn the rules of watermark embedding and extraction, resulting in a fully automated and optimized watermarking system. 
